A Hybrid Data-driven Deep Learning Technique for Fluid-Structure Interaction

This paper is concerned with the development of a hybrid data-driven technique for unsteady fluid-structure interaction systems. The proposed data-driven technique combines the deep learning framework with a projection-based low-order modeling. While the deep learning provides low-dimensional approximations from datasets arising from black-box solvers, the projection-based model constructs the low-dimensional approximations by projecting the original high-dimensional model onto a low-dimensional subspace. Of particular interest of this paper is to predict the long time series of unsteady flow fields of a freely vibrating bluff-body subjected to wake-body synchronization. We consider convolutional neural networks (CNN) for the learning dynamics of wake-body interaction, which assemble layers of linear convolutions with nonlinear activations to automatically extract the low-dimensional flow features. Using the high-fidelity time series data from the stabilized finite element Navier-Stokes solver, we first project the dataset to a low-dimensional subspace by proper orthogonal decomposition (POD) technique. The time-dependent coefficients of the POD subspace are mapped to the flow field via a CNN with nonlinear rectification, and the CNN is iteratively trained using the stochastic gradient descent method to predict the POD time coefficient when a new flow field is fed to it. The time-averaged flow field, the POD basis vectors, and the trained CNN are used to predict the long time series of the flow fields and the flow predictions are quantitatively assessed with the full-order (high-dimensional) simulation data. The proposed POD-CNN model based on the data-driven approximation has a remarkable accuracy in the entire fluid domain including the highly nonlinear near wake region behind a freely vibrating bluff body.

==> Nomenclature.tex <==
\makeatletter
\newif\if@checkentries
\renewenvironment{nomenclature}[1][]
 {\if\relax\detokenize{#1}\relax
    \@checkentriesfalse
  \else
    \settowidth{\@tempdima}{#1\quad}%
    \@checkentriestrue
  \fi
  \def\entry##1##2{%
    \sbox\@tempboxa{##1\quad}%
    \if@checkentries
      \ifdim\wd\@tempboxa>\@tempdima
        \@latex@warning{Entry `\unexpanded{##1}' is wider}%
        \@tempdima=\wd\@tempboxa
      \fi
    \else
      \@tempdima=\wd\@tempboxa
    \fi
    \hangindent\@tempdima
    \noindent\makebox[\@tempdima][l]{##1}\ignorespaces##2\par}%
    \section*{NOMENCLATURE}}
 {\par\addvspace{12pt}}
\makeatother
